Parallel and (Nearly) Work-Efficient Dynamic Programming

The idea of dynamic programming (DP), proposed by Bellman in the 1950s, is one of the most important algorithmic techniques. However, in parallel, many fundamental and sequentially simple problems become more challenging, and open to a (nearly) work-efficient solution (i.e., the work is off by at most a polylogarithmic factor over the best sequential solution). In fact, sequential DP algorithms employ many advanced optimizations such as decision monotonicity or special data structures, and achieve better work than straightforward solutions. Many such optimizations are inherently sequential, which creates extra challenges for a parallel algorithm to achieve the same work bound. The goal of this paper is to achieve (nearly) work-efficient parallel DP algorithms by parallelizing classic, highly-optimized and practical sequential algorithms. We show a general framework called the Cordon Algorithm for parallel DP algorithms, and use it to solve several classic problems. Our selection of problems includes Longest Increasing Subsequence (LIS), sparse Longest Common Subsequence (LCS), convex/concave generalized Least Weight Subsequence (LWS), Optimal Alphabetic Tree (OAT), and more. We show how the Cordon Algorithm can be used to achieve the same level of optimization as the sequential algorithms, and achieve good parallelism. Many of our algorithms are conceptually simple, and we show some experimental results as proofs-of-concept.

==> alg/cordon.tex <==
\begin{algorithm}[t]
\small
\caption{The Framework of \ouralgo{}\label{alg:ours}}
\SetKwProg{myfunc}{Function}{}{}
\SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
\SetKwFor{mystruct}{Struct}{}{}
\SetKwFor{pardo}{In Parallel:}{}{}
Mark all states as tentative and initialize them by the boundary condition\\
\While{$\exists$ tentative states} {
  If a tentative state $i$ can be relaxed by another tentative state $j$, put a \sentinel{} on state $i$. 
  A state is \textbf{ready} if there is no \sentinel{} on any of its ancestors (including itself). \\
  For all ready states, use their DP values to relax the DP values of all of its successors.\\
  Mark all ready states as finalized; Clear all the sentinels.
}
\end{algorithm} 
